Tracking the Best Expert Privately

We design differentially private algorithms for the problem of prediction with expert advice under dynamic regret, also known as tracking the best expert. Our work addresses three natural types of adversaries, stochastic with shifting distributions, oblivious, and adaptive, and designs algorithms with sub-linear regret for all three cases. In particular, under a shifting stochastic adversary where the distribution may shift $S$ times, we provide an $\epsilon$-differentially private algorithm whose expected dynamic regret is at most $O\left( \sqrt{S T \log (NT)} + \frac{S \log (NT)}{\epsilon}\right)$, where $T$ and $N$ are the epsilon horizon and number of experts, respectively. For oblivious adversaries, we give a reduction from dynamic regret minimization to static regret minimization, resulting in an upper bound of $O\left(\sqrt{S T \log(NT)} + \frac{S T^{1/3}\log(T/\delta) \log(NT)}{\epsilon^{2/3}}\right)$ on the expected dynamic regret, where $S$ now denotes the allowable number of switches of the best expert. Finally, similar to static regret, we establish a fundamental separation between oblivious and adaptive adversaries for the dynamic setting: while our algorithms show that sub-linear regret is achievable for oblivious adversaries in the high-privacy regime $\epsilon \le \sqrt{S/T}$, we show that any $(\epsilon, \delta)$-differentially private algorithm must suffer linear dynamic regret under adaptive adversaries for $\epsilon \le \sqrt{S/T}$. Finally, to complement this lower bound, we give an $\epsilon$-differentially private algorithm that attains sub-linear dynamic regret under adaptive adversaries whenever $\epsilon \gg \sqrt{S/T}$.

==> algorithm.tex <==
\section{Adaptive Algorithm Stochastic Case (Fixed $\P$)}
\label{sec:alg_stoc}

In this section we first propose an algorithm that is adaptive to the underlying preference structure $\P$. More precisely, the algorithm can adapt itself to the \tot \, structure if $\P$ respects total ordering, yielding an optimal regret bound of $\tO\big( \sum_{k = 1}^{K} \frac{\log T}{\Delta_i} \big)$. On the other hand, under only \cw \, structure it yields a regret guarantee of $\tO\big( \sum_{k = 1}^{K} K\frac{\log T}{\Delta_i} \big)$, which is tight up to a constant factor of $K$ (more details in Rem. \ref{rem:opt_vs_reg}).

\subsection{Algorithm description: Main Ideas}



{\bf High-level idea behind algorithm design.} The algorithm we propose (\algfewf) is based on using an $(\epsilon,\delta)$-PAC-algorithm known to have (expected) termination time bounded in terms of $\epsilon$ and $\delta$ (a `worst' case termination guarantee not necessarily dependent on instance parameters) as an underlying black-box subroutine. The wrapper algorithm uses the black-box repeatedly, with successively more stringent values of $\epsilon$ and $\delta$, to eliminate suboptimal arms in a phased manner. The termination analysis of the algorithm shows that any suboptimal arm $i \in [n]\sm \{1\}$ survives for about  $O\Big(\frac{1}{\Delta_i^2}\ln \frac{k}{\delta}\Big)$ rounds before being eliminated, which leads to the desired bound of $O\bigg(\sum_{i=2}^{n}\frac{1}{\Delta_i^2}\ln \frac{k}{\delta}\bigg)$ on algorithm's run time performance (with high probability $(1-\delta)$) (Thm. \ref{thm:sc_fewf}).

%\textbf{Main Idea.} The crucial idea behind bringing out this problem dependent complexity term $(\Delta_i)$ lies in using a $(\epsilon,\delta)$-PAC routine with gradually diminishing adaptive $\epsilon$ values, and judge the competency of rest of surviving arms with respect to the $(\epsilon,\delta)$-PAC winner. 
\vspace{-2pt}
{\bf Algorithm description.} The \algm\, algorithm we propose (Alg. \ref{alg:fewf}) runs in phases indexed by $s = 1,2,\ldots$, where each phase $s$ comprises of the following steps.

{\bf Step 1: Finding a good reference item.} It first calls an $(\epsilon_s,\delta_s)$-PAC subroutine (described in Sec. \ref{sec:alg_epsdel} for completeness) with $\epsilon_s = \frac{1}{2^{s+2}}$ and $\delta_s = \frac{\delta}{120s^3}$ to obtain a `reasonably good item' $b_s$---an item that is likely within an $\epsilon_s$ margin of the \bi\, with probability at least $(1-\delta_s)$) and thus a potential \bi. For this we design a new sequential elimination-based algorithm (Alg. \ref{alg:epsdel} in Appendix \ref{app:wiub_div}),  and argue that it finds such a $(\epsilon_s,\delta_s)$-PAC `good item' with {\em instance-dependent} sample complexity (Thm. \ref{lem:up_algep}), which is crucial in the overall analysis. This is an improvement upon the instance-agnostic Algorithm 6 of \cite{SGwin18} whose sample complexity guarantee is not strong enough to be used along with the wrapper. 
%, which otherwise would have blew up the total sample complexity of the main procedure.
%This pivot finding step is crucial proposed

{\bf Step 2: Benchmarking items against the reference item.} After obtaining a candidate good item, the algorithm pairs up the rest of the surviving arms with this good `probe' item $b_s$ and plays each pair multiple times (up to $t_s =  \frac{4}{\epsilon_s^2}\ln \frac{1}{\delta_s} $ rounds), where $\thetsh$ denotes a 'near-accurate' relative score estimate of the \pl\, model for the set $\cB_b$--we use the subroutine \algs\, for estimating $\thetsh$ (see Alg. \ref{alg:algs}, Thm. \ref{thm:algs} in Appendix \ref{app:subrout}). From the winner data obtained in this process, it updates the empirical pairwise win count $w_i$ of each item within any batch $\cB_b$ by applying a rank-breaking idea (see Alg. \ref{alg:updt_win}, Appendix \ref{app:subrout}) .% (the \rb\, subroutine, Algorithm \ref{alg:updt_win}, Appendix \ref{app:alg_fewf}).

{\bf Step 3: Discarding items weaker than the reference item.} Finally, from each group $\cB_b$, the algorithm eliminates all arms whose empirical pairwise win frequency  over the probe item $b_s$ is less than $\frac{1}{2} - \epsilon_s$ (i.e. $\forall i \in \cB_b$ for which $\hat{p}_{i b_s}< \frac{1}{2} - \epsilon_s$, $\hat{p}_{i j}$ being the empirical pairwise preference of item $i$ over $j$ obtained via \rb). The next phase then begins, unless there is only one surviving item left, which is output as the candidate \bi. 

%The details of the $(\epsilon,\delta)$-PAC algorithm is described in Sec. \ref{sec:alg_epsdel}. But before that we briefly describe the concept of \rb\, update below:

\noindent
\textbf{(1). \algep\, subroutine:} Given $\epsilon, \delta \in (0,1)$, this finds an $(\epsilon, \delta)$-\bi\, in $O\Big(\frac{\thetk}{\epsilon^2}\ln \frac{k}{\delta}\Big)$ samples, where $\thetk=\hspace{-8pt} \underset{S \subseteq [n] \mid |S|=k}{\max} \sum_{i \in S}\theta_i$ (See Alg. \ref{alg:epsdel}, Thm. \ref{lem:up_algep} in Appendix \ref{app:wiub_div}). 

\vspace{-5pt}
\begin{center}
\begin{algorithm}[H]
   \caption{\textbf{\algm}}
   \label{alg:algm}
	\begin{algorithmic}[1]
   \STATE {\bfseries input:} Set of items: $[n]$, Confidence term $\delta > 0$, $n_{ij}(1) \leftarrow 0 ~\forall i,j \in [n]$
   \STATE {\bfseries init:}  $\cA_0 \leftarrow [n]$, $t \leftarrow 1$, $s \leftarrow 1$,  
   \WHILE {$|\cA_{s-1}| > 1$}
   \STATE Set $\epsilon_s = \frac{1}{2^{s+2}}$, $\delta_s = \frac{\delta}{120s^3}$
   \STATE $n_i \leftarrow 0$ for all $i \in \cA_{s-1} \sm \{b_s\}$
   \STATE $b_s \leftarrow $ \algep$(\cA_{s-1},k,1,\epsilon_s,\delta_s)$ 
   
   \REPEAT 
   \STATE Play $(\ell_t,r_t) \in \text{argmin}_{i,j \in \cA_{t-1}} \{ n_{ij}(t)\}$
   \STATE For every pair $i,j \in \cA_{t-1}$ define
   \[
   u_{ij}(t) = \hat p_{ij}(t) + \sqrt{\frac{\alpha \log t}{n_{ij}(t)}}
   \]
   \STATE $n_{i_t,j_t}(t+1) \leftarrow n_{i_t,j_t}(t)+1$
   \STATE Choose $k_t \in \text{argmin}_{i \in \cA_{t-1}} \{ n_{ij}(t)\}$
   \STATE Set $\ell_t' \leftarrow b_s$, $r_t' \leftarrow k_t$ and play $(\ell_t',r_t')$
   \STATE if   %Check for RR
   \STATE %Check for Wrapper
   
   \STATE $t \leftarrow t+1$
   
   \UNTIL {(A),(B), or (C) holds good} 
   
   \STATE $\cA_{t+1} = \cA_t \backslash \big\{i \in \cA_t: \exists j \in A_t \ \text{s.t.}\quad  u_{ij}(t) < \frac{1}{2}\big\}$ \,
   
   $\sigma_1\ldots \sigma_{t_s}, ~\forall i,j \in \cB_b$  
   \STATE $\hp_{ij} := \frac{w_{ij}}{w_{ij} + w_{ji}}$ for all $i,j \in \cB_b$
   \STATE \textbf{If} $\exists i \in \cB_b$ s.t. $\hp_{ib_s} < \frac{1}{2} - \epsilon_s$, \textbf{then} $\cA_s \leftarrow \cA_{s} \cup \{i\}$
%   \ENDFOR
	\STATE $s \leftarrow s + 1$
  \ENDWHILE

   \STATE {\bfseries output:} The item remaining in $\cA_s$ 
	\end{algorithmic}
\end{algorithm}
\vspace{-5pt}
\end{center}


\begin{center}
	\begin{algorithm}[H]
		\caption{\textbf{\algep} }
		\label{alg:edpac}
		\begin{algorithmic}[1]
			\STATE {\bfseries Input:} 
			\STATE ~~~ Set of items: $[n]$
			\STATE ~~~ Error bias: $\epsilon >0$, and confidence parameter: $\delta >0$
			\STATE {\bfseries Initialize:} 
			\STATE ~~~ $S \leftarrow [n]$, $\epsilon_0 \leftarrow \frac{\epsilon}{8}$, and $\delta_0 \leftarrow \frac{\delta}{2}$  
			\WHILE{$\ell = 1,2, \ldots$}
			\STATE Set $\delta_\ell \leftarrow \frac{\delta_{\ell-1}}{2}, \epsilon_\ell \leftarrow \frac{3}{4}\epsilon_{\ell-1}$
			\FOR {$g = 1,2, \cdots G$}
			\STATE $\thetg \leftarrow $ \algs$\big(\cG_g,b,\delta_\ell \big)$
			\FOR {$\tau = 1, 2, \ldots t := \left\lceil \frac{32}{\epsilon_l^2} \ln \frac{4}{\delta_\ell} \right\rceil$  }
			\STATE Play the set $\cG_g$ (one round of battle)
			\STATE Receive feedback: The top-$m$ ranking $\bsigma \in \bSigma_{\cG_{g}}^m$ 
			\STATE Update win-count $w_{ij}$ of each item pair $i,j \in \cG_g$
			\ENDFOR 
			%   	\STATE $B_\ell \leftarrow \text{argmax}\{ i \in \cA \mid  \sum_{j \in \cA\setminus\{i'\}}~\1\big(w_{ij} \ge w_{ji}\big) \}$  
			\STATE Estimate pairwise win probabilities: $\forall i,j \in \cG_g \; \hat p_{i,j} = \frac{w_{ij}}{w_{ij}+w_{ji}}$ if $w_{ij}+w_{ji} > 0$, $\hat p_{i,j} = \frac{1}{2}$ otherwise 
			\STATE If $\exists i \in \cG_g$ such that $\hp_{i j} + \frac{\epsilon_\ell}{2} \ge \frac{1}{2}, \, \forall j \in \cG_g$, then set $c_g \leftarrow i$, else select $c_g \leftarrow$ uniformly at random from $\cG_g$. Set $S \leftarrow S \setminus \left( \cG_g \setminus  \{c_g\}\right)$
			\ENDFOR
			\STATE $S \leftarrow S \cup \cR_\ell$
			\IF{$(|S| == 1)$}
			\STATE Break (out of the {\bf while} loop)
			\ELSIF{$|S|\le k$}
			\STATE $S' \leftarrow $ Randomly sample $k-|S|$ items from $[n] \setminus S$, and set $S \leftarrow S \cup S'$, $\epsilon_\ell \leftarrow \frac{2\epsilon}{3}$, $\delta_\ell \leftarrow {\delta}$  
			%	\STATE Initialize pairwise (empirical) win-count $w_{ij} \leftarrow 0$, for each item pair $i,j \in S$
			%	\FOR {$\tau = 1, 2, \ldots t\,(:= \frac{k}{m\epsilon_\ell^2}\ln \frac{2k}{\delta_\ell})$}
			%   	\STATE Play the set $S$ (one round of battle)
			%   	\STATE Receive TR feedback: $\bsigma \in \bSigma_{S^\tau_{m}}$, where $S^\tau_{m} \subseteq S$ such that $|S^\tau_{m}| = m$ 
			%   	\STATE Update win-count $w_{ij}$ of each item pair $i,j \in S$ using \algupdt$(S,\bsigma)$
			%   	\ENDFOR
			%   	\STATE Define $\hat p_{i,j} = \frac{w_i}{w_i+w_j}, \, \forall i,j \in S$
			%   	\STATE \textbf{If} $\exists i \in \cG_g$ such that $\hp_{i j} + \frac{\epsilon}{2} \ge \frac{1}{2}, \, \forall j \in \cG_g$, \textbf{then} set $c_g \leftarrow i$, \textbf{else} select $c_g \leftarrow$ uniformly at random from $\cG_g$, and  Break (go out of the while loop)
			%  \ELSE
			\ENDIF
			\STATE Divide $S$ into $G: = \big \lceil \frac{|S|}{k} \big \rceil$ sets $\cG_1, \cdots \cG_G$ such that $\cup_{j = 1}^{G}\cG_j = S$, $\cG_{j} \cap \cG_{j'} = \emptyset, ~\forall j,j' \in [G], \, |G_j| = k,\, \forall j \in [G-1]$. \textbf{If} $|\cG_{G}| < k$, \textbf{then} set $\cR_{\ell+1} \leftarrow \cG_G$  and $G = G-1$, \textbf{Else} $\cR_1 \leftarrow \emptyset$.
			
			\ENDWHILE
			%   \UNTIL{$(S == \emptyset)$}
			\STATE {\bfseries Output:} $r_*$, the single item remaining in $S$ %: an $\epsilon$-optimal item
		\end{algorithmic}
	\end{algorithm}
	\vspace{-10pt}
\end{center}

\begin{restatable}[\algfewf: Sample Complexity for $(0,\delta)$-PAC Guarantee for \tf]{thm}{scalgfetf}
	\label{thm:sc_fetf}
	With probability at least $(1-\delta)$, \algfewf\, (Algorithm \ref{alg:fewf}) returns the \bi\,  with sample complexity $N_\cA(0,\delta) = O\bigg(\frac{\thetk}{k}\sum_{i = 2}^n\max\Big( 1, \frac{1}{m\Delta_i^2}\Big) \ln\frac{k}{\delta}\Big(\ln \frac{1}{\Delta_i}\Big)\bigg)$. %where $\thetk: = \arg \max_{S \subseteq [n] \mid |S|=k} \sum_{i \in S}\theta_i$.
	%\red{To be corrected.}
\end{restatable}

\begin{rem}
	Following the similar procedure as argued in Sec. \ref{sec:alg_epsdel}, one can easily derive an $(\epsilon,\delta)$-PAC version of \algfetf\, as well, and a similar  guarantee as that of Thm. \ref{thm:sc_fewfep} with a reduction factor $1/m$. We omit the details in the interest of space.
\end{rem}

\newpage %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\begin{proof}
	As argued, the main idea behind the $\frac{1}{m}$ factor improvement in the sample complexity w.r.t \wf\, (as proved in Thm. \ref{thm:sc_fewf}), lies behind using \rb \, updates (see Alg. \ref{alg:updt_win}) to the general \tf. This actually gives rise to $O(m)$ times additional number of pairwise preferences in comparison to \wf\, which is why in this case it turns out to be sufficient to sample any batch $\cB_b, \forall b \in [B_s]$ for only  $O\big( \frac{1}{m} \big)$ times compared to the earlier case---precisely the reason behind $\frac{1}{m}$-factor improved sample complexity of \algfewf\, for \tf. The rest of the proof argument is mostly similar to that of Thm. \ref{thm:sc_fewf}. We provide the detailed analysis below for the sake of completeness.
	
	%The proof is based on the following four main observations:
	%\begin{enumerate}
	%\item The \bi\, $a^*$ (i.e. item $1$ in our case) is likely to beat the ($\epsilon_s,\delta_s$)-PAC item by sufficiently high margin, for any sub-phase $s= 1,2\ldots$, and hence is never discarded (see Lem. \ref{lem:bistays}).
	%\item With high probability the set of suboptimal items get discarded at a fixed rate once played for sufficiently long duration (see Lem. \ref{lem:nbigoes}).
	%\item The number of occurrences of any sub-optimal item $i$ before it gets discarded is proportional to $O\Big(\frac{1}{\Delta_i^2}\Big)$ which yields the desired sample complexity of the algorithm (see Lem.\ref{lem:sc_item}).
	%\item Lastly we show in Lem. \ref{lem:sc_bbox} that the additional sample complexity incurred due to invoking the subroutine \algep\, at every sub-phase $s$ is orderwise same as the sample complexity incurred by \algfewf\, in the rest of the sub-phase, due to which \algep\, does  contribute to the overall sample complexity of the algorithm modulo some constant factors.
	%\end{enumerate}
	
	We start by proving the correctness of the algorithm, i.e. with high probability $(1-\delta)$, \algfewf\, indeed returns the \bi\,, i.e. item $1$ in our case. Towards this we first prove the following two lemmas: Lem. \ref{lem:bistaystf} and Lem. \ref{lem:nbigoestf}, same as what was derived for Thm. \ref{thm:sc_fewf} as well---However it is important to note that its is due to the \tf\, feedback the exact same guarantees holds in this case as well, even with a $m$-times lesser observed samples.
	
	\begin{restatable}[]{lem}{bistaystf}
		\label{lem:bistaystf}
		With high probability of at least $(1-\frac{\delta}{20})$, item $1$ is never eliminated, i.e. $1 \in \cA_s$ for all sub-phase $s$. More formally, at the end of any sub-phase $s= 1,2,\ldots$, $\hp_{1b_s} > \frac{1}{2} - \epsilon_s$.
	\end{restatable}
	
	\begin{proof}
		Firstly note that at any sub-phase $s$, each batch $b \in B$ within that phase is played for $t_s = \frac{2\thetk}{m\epsilon_s^2}\ln \frac{k}{\delta_s}$ rounds. Now consider the batch $\cB \owns 1$ at any phase $s$. Clearly $b_s \in \cB$ too. Again since $b_s$ is returned by Alg. \ref{alg:epsdel}, by Thm. \ref{lem:up_algep} we know that with probability at least $(1-\delta_s)$, $p_{b_s1} > \frac{1}{2} - \epsilon_s \, \implies \theta_{b_s} > \theta_1 - 4\epsilon$. This further implies $\theta_{b_s} \ge \theta_1 - \frac{1}{2} = \frac{1}{2}$ (since we assume $\theta_1 = 1$, and at any $s,\, \epsilon_s < \frac{1}{8}$). Moreover by Lem. \ref{lem:algs}, we have $\thetsh \ge \frac{\theta_{b_s} +\thets }{\theta_{b_s}} > \frac{\thets + 1}{2}$ (recall we denote $S = \cB_b \sm \{b_s\}$)
		
		Now let us define $w_i$ as number of times item $i \in \cB$ was returned as the winner in $t_s$ rounds and $i_\tau$ be the winner retuned by the environment upon playing $\cB$ for the $\tau^{th}$ round, where $\tau \in [t_s]$.
		Then clearly $Pr(\{1 \in \sigma_\tau\}) = \sum_{j = 1}^{m}Pr\big( \sigma_\tau(j) = 1 \Big) \ge \frac{m\theta_{1}}{\sum_{j \in \cB}\theta_j} = \frac{m}{\theta_{b_s} + \thets} \ge \frac{m}{1+ \thets}, \, \forall \tau \in [t_s]$, as $1 := \arg \max_{i \in \cB}\theta_i$. Hence $\E[w_{1}] = \sum_{\tau = 1}^{t_s}\E[\1(i_\tau = 1)] = \frac{mt_s}{\theta_{b_s} + \thets} \ge \frac{mt_s}{(1+\thets)}$. 
		Now assuming $b_s$ to be indeed an $(\epsilon_s,\delta_s)$-PAC \bi\, and the bound of Lem. \ref{lem:algs} to hold good as well, applying multiplicative Chernoff-Hoeffdings bound on the random variable $w_{1}$, we get that for any $\eta \in (\sqrt{2}\epsilon_s,1]$, 
		
		\begin{align*}
			Pr\Big( w_{1} \le (1-\eta)\E[w_{1}] \Big) & \le \exp\bigg(- \frac{\E[w_{1}]\eta^2}{2}\bigg) \le \exp\bigg(- \frac{mt_s\eta^2}{2(1+\thets)}\bigg) \\
			& = \exp\bigg(- \frac{2\thetsh\eta^2}{2m\epsilon_s^2(1+\thets)}\ln \frac{k}{\delta_s}\bigg)\\
			&\stackrel{(a)}{\le} \exp\bigg(- \frac{2(\thets+1)\eta^2}{4\epsilon_s^2(1+\thets)}\ln \frac{k}{\delta_s}\bigg)\\
			& \le \exp\bigg(- \frac{\eta^2}{2\epsilon_s^2} \ln \bigg( \frac{k}{\delta_s} \bigg) \bigg) \le \exp\bigg(- \ln \bigg( \frac{k}{\delta_s} \bigg) \bigg) = \frac{\delta_s}{k},
		\end{align*}
		where $(a)$ holds since we proved $\thetsh \ge \frac{\theta_{b_s} +\thets }{\theta_{b_s}} > \frac{\thets + 1}{2}$, and the last inequality holds as $\eta > \epsilon_s\sqrt{2}$.
		
		In particular, note that $\epsilon_s \le \frac{1}{8}$ for any sub-phase $s$, due to which we can safely choose $\eta = \frac{1}{2}$ for any $s$, which gives that with probability at least $\big(1-\frac{\delta_s}{k}\big)$,  $w_{1} > (1-\frac{1}{2})\E[w_{1}] > \frac{mt_s}{2(\theta_{b_s}+\thets)}$, for any subphase $s$.
		
		%====================
		
		Thus above implies that with probability atleast $(1-\frac{\delta_s}{k})$, after $t_s$ rounds we have $w_{1b_s} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)} \implies w_{1b_s} + w_{b_s1} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)}$. Let us denote  $n_{1b_s} = w_{1b_s} + w_{b_s1}$. Then the probability of the event:
		
		\begin{align*}
			Pr\Bigg(  \hp_{1 b_s} & < \frac{1}{2} - \epsilon_s  ,  n_{1 b_s} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)}  \Bigg)
			= Pr\Bigg( \hp_{1 b_s} - \frac{1}{2} < - \epsilon_s  ,  n_{1 b_s} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)} \Bigg)\\
			& \le Pr\Bigg( \hp_{1 b_s} - p_{1 b_s} < - \epsilon_s  ,  n_{1 b_s} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)} \Bigg) ~~~(\text{as } \p_{1 b_s} > \frac{1}{2})\\
			& \stackrel{(a)} \le \exp\Big( -2\frac{mt_s}{2(\theta_{b_s}+\thets)}\big({\epsilon_s}\big)^2 \Big) \\
			& \le \exp\Big( -\frac{2m(\theta_{b_s} + \thets)}{m\epsilon_s^2\theta_{b_s}(\theta_{b_s}+\thets)}\big({\epsilon_s}\big)^2 \Big) 
			\le \frac{\delta_s}{k},
		\end{align*}
		
		where the last inequality $(a)$ follows from Lem. \ref{lem:pl_simulator} for $\eta = \epsilon_s$ and $v = \frac{t_s}{2k}$.
		
		Thus under the two assumptions that (1). $b_s$ is indeed an $(\epsilon_s,\delta_s)$-PAC \bi\, and (2). the bound of Lem. \ref{lem:algs} holds good, combining the above two claims, at any sub-phase $s$, we have
		
		\begin{align*}
			& Pr\Bigg(  \hp_{1 b_s} < \frac{1}{2} - \epsilon_s\Bigg)\\
			& = 
			Pr\Bigg(  \hp_{1 b_s} < \frac{1}{2} - \epsilon_s  ,  n_{1 b_s} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)}  \Bigg) + Pr\Bigg(  \hp_{1 b_s} < \frac{1}{2} - \epsilon_s  ,  n_{1 b_s} < \frac{mt_s}{2(\theta_{b_s}+\thets)}  \Bigg)\\
			& \le \frac{\delta_s}{k} + Pr\Bigg( n_{1 b_s} < \frac{mt_s}{2(\theta_{b_s}+\thets)}  \Bigg) \le \frac{2\delta_s}{k} \le \delta_s ~~~(\text{since } k \ge 2)\\
		\end{align*}
		
		Moreover from Thm. \ref{lem:up_algep} and Lem. \ref{lem:algs} we know that the above two assumptions hold with probability at least $(1-2\delta_s)$. Then taking union bound over all sub-phases $s = 1,2, \ldots$, the probability that item $1$ gets eliminated at any round:
		
		\begin{align*}
			Pr\Bigg( \exists s = 1,2, \ldots \text{ s.t. } \hp_{1 b_s} < \frac{1}{2} - \epsilon_s \Bigg) & = \sum_{s = 1}^{\infty}{3\delta_s} = \sum_{s = 1}^{\infty}\frac{3\delta}{120s^3} \le \frac{\delta}{40}\sum_{s = 1}^{\infty}\frac{1}{s^2} \le \frac{\delta}{40}\frac{\pi^2}{6} \le \frac{\delta}{20},
		\end{align*}
		where the first inequality holds since $k \ge 2$.
	\end{proof}
	Recall the notations introduced in the proof of Thm. \ref{thm:sc_fewf}: $\Delta_i = \theta_1-\theta_i$ (Sec. \ref{sec:prb_setup}), $\Delta_{\min} = \min_{i \in [n]\sm\{1\}}\Delta_i$.
	Further $[n]_r := \{ i \in [n] : \frac{1}{2^r} \le \Delta_i < \frac{1}{2^{r-1}} \}$, and $\cA_{r,s}$, i.e. $\cA_{r,s} = [n]_r \cap \cA_s$, for all $s = 1,2, \ldots$.
	Then in this case again we claim:
	
	\begin{restatable}[]{lem}{nbigoestf}
		\label{lem:nbigoestf}
		Assuming that the best arm $1$ is not eliminated at any sub-phase $s = 1,2,\ldots$, then with probability at least $(1-\frac{19\delta}{20})$, for any sub-phase $s \ge r$, $|\cA_{r,s}| \le \frac{2}{19}|\cA_{r,s-1}|$, for any $r = 0,1,2,\ldots \log_2 (\Delta_{\min})$. 
	\end{restatable}
	
	
	\begin{proof}
		Consider any sub-phase $s$, and let us start by noting some properties of $b_s$. Note that by Lem. \ref{lem:up_algep}, with high probability $(1-\delta_s)$, $p_{b_s 1} > \frac{1}{2} - \epsilon_s$. Then this further implies
		
		\begin{align*}
			p_{b_s 1} > \frac{1}{2} - \epsilon_s & \implies \frac{(\theta_{b_s} - \theta_1)}{2(\theta_{b_s} + \theta_1)} > -\epsilon_s\\
			& \implies (\theta_{b_s} - \theta_1) > -2\epsilon_s(\theta_{b_s} + \theta_1) > -4\epsilon_s ~~(\text{as} ~\theta_i \in (0,1)\, \forall i \in [n]\sm\{1\}) 
		\end{align*}  
		
		So we have with probability atleast $(1-\delta_s)$,  $\theta_{b_s} > \theta_1 - 4\epsilon_s = \theta_1 - \frac{1}{2^s}$. 
		
		Now consider any fixed $r = 0,1,2,\ldots \log_2(\Delta_{\min})$. Clearly by definition, for any item $i \in [n]_r$, $\Delta_i = \theta_1 - \theta_i > \frac{1}{2^r}$.
		Then combining the above two claims, we have for any sub-phase $s \ge r$, $\theta_{b_s} > \theta_1 - \frac{1}{2^s} \ge \theta_i + \frac{1}{2^r} - \frac{1}{2^s} > 0 \implies p_{b_si} > \frac{1}{2}$, at any $s \ge r$.
		Moreover note that for any $s \ge 1$, $\epsilon_s > \frac{1}{8}$, so that implies $\theta_{b_s} > \theta_1 - 4\epsilon_s > \frac{1}{2}$.
		
		%====================
		
		Recall that at any sub-phase $s$, each batch within that phase is played for $t_s = \frac{2\thetk}{m\epsilon_s^2}\ln \frac{k}{\delta_s}$ many rounds. Now consider any batch such that $\cB \owns i$ for any $i \in [n]_r$. Of course $b_s \in \cB$ as well, and note that we have shown $p_{b_si} > \frac{1}{2}$ with high probability $(1-\delta_s)$. 
		
		Same as Lem. \ref{lem:bistays}, let us again define $w_i$ as number of times item $i \in \cB$ was returned as the winner in $t_s$ rounds, and $i_\tau$ be the winner retuned by the environment upon playing $\cB$ for the $\tau^{th}$ rounds, where $\tau \in [t_s]$.
		Then given $\theta_{b_s} > \frac{1}{2}$ (as derived earlier), clearly $Pr(\{b_s \in \sigma_\tau\}) = \sum_{j = 1}^{m}Pr\big( \sigma_\tau(j) = b_s \Big) \ge \sum_{j = 0}^{m-1}\frac{\theta_{b_s}}{(\theta_{b_s} + \thets)} = \frac{m\theta_{b_s}}{\theta_{b_s} + \thets}, \, \forall \tau \in [t_s]$. Hence $\E[w_{b_s}] = \sum_{\tau = 1}^{t_s}\E[\1(i_\tau = b_s)] = \frac{m\theta_{b_s}t_s}{(\theta_{b_s} + \thets)}$. 
		Now applying multiplicative Chernoff-Hoeffdings bound on the random variable $w_{b_s}$, we get that for any $\eta \in (\sqrt 2\epsilon_s,1]$, 
		
		\begin{align*}
			Pr\Big( w_{b_s} & \le (1-\eta)\E[w_{b_s}] \mid \theta_{b_s} > \frac{1}{2}, \thetsh > \frac{(\theta_{b_s} + \thets)}{\theta_{b_s}} \Big)\\
			& \le \exp\bigg(- \frac{\E[w_{b_s}]\eta^2}{2}\bigg) \le \exp\bigg(- \frac{m\theta_{b_s}t_s\eta^2}{2(\theta_{b_s} + \thets)}\bigg) \\
			& \le \exp\bigg(- \frac{\eta^2}{2\epsilon_s^2} \ln \bigg( \frac{k}{\delta_s} \bigg) \bigg) \le \exp\bigg(- \ln \bigg( \frac{k}{\delta_s} \bigg) \bigg) = \frac{\delta_s}{k},
		\end{align*}
		where the last inequality holds as $\eta > \sqrt 2\epsilon_s$.
		So as a whole, for any $\eta \in (\sqrt 2\epsilon_s,1]$,
		
		\begin{align*}
			& Pr\Big( w_{b_s} \le (1-\eta)\E[w_{b_s}] \Big)\\
			& \le Pr\Big( w_{b_s} \le (1-\eta)\E[w_{b_s}] \mid \theta_{b_s} > \frac{1}{2}, \thetsh > \frac{(\theta_{b_s} + \thets)}{\theta_{b_s}}  \Big)Pr\Big(\theta_{b_s} > \frac{1}{2}\Big) + Pr\Big(\theta_{b_s} < \frac{1}{2},\thetsh > \frac{(\theta_{b_s} + \thets)}{\theta_{b_s}} \Big)\\ 
			& \le \frac{\delta_s}{k} + 2\delta_s
		\end{align*}
		
		In particular, note that $\epsilon_s < \frac{1}{8}$ for any  sub-phase $s$, due to which we can safely choose $\eta = \frac{1}{2}$ for any $s$, which gives that with probability at least $\big(1-\frac{\delta_s}{k}\big)$,  $w_{b_s} > (1-\frac{1}{2})\E[w_{b_s}] > \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})}$, for any subphase $s$.
		
		Thus above implies that with probability at least $(1-\frac{\delta_s}{k}-2\delta_s)$, after $t_s$ rounds we have $w_{b_si} \ge \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})} \implies w_{ib_s} + w_{b_si} \ge \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})}$. Let us denote  $n_{ib_s} = w_{ib_s} + w_{b_si}$. Then the probability that item $i$ is not eliminated at any sub-phase $s \ge r$ is:
		
		\begin{align*}
			Pr\Bigg(  \hp_{i b_s} > \frac{1}{2} & - \epsilon_s  ,  n_{i b_s} \ge \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})}  \Bigg)
			= Pr\Bigg( \hp_{i b_s} - \frac{1}{2} > - \epsilon_s  ,  n_{i b_s} \ge \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})} \Bigg)\\
			& \le Pr\Bigg( \hp_{i b_s} - p_{i b_s} > - \epsilon_s  ,  n_{1 b_s} \ge \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})}\Bigg) ~~~(\text{as } \p_{i b_s } < \frac{1}{2})\\
			& \stackrel{(a)}\le \exp\Big( -2\frac{mt_s}{2(\thets + \theta_{b_s})}\big({\epsilon_s}\big)^2 \Big)\\
			& \le \exp\Big( -2\frac{m(\thets + \theta_{b_s})}{2m\theta_{b_s}(\thets + \theta_{b_s})}\big({\epsilon_s}\big)^2 \ln \frac{\delta_s}{k}\Big) \le \frac{\delta_s}{k},
		\end{align*}
		
		where $(a)$ follows from Lem. \ref{lem:pl_simulator} for $\eta = \epsilon_s$ and $v = \frac{t_s}{2k}$.
		
		Now combining the above two claims, at any sub-phase $s$, we have:
		
		\begin{align*}
			Pr\Bigg(  \hp_{i b_s} > \frac{1}{2} - \epsilon_s\Bigg) & = 
			Pr\Bigg(  \hp_{i b_s} > \frac{1}{2} - \epsilon_s  ,  n_{i b_s} \ge \frac{t_s}{4k}  \Bigg) + Pr\Bigg(  \hp_{i b_s} > \frac{1}{2} - \epsilon_s  ,  n_{i b_s} < \frac{t_s}{4k}  \Bigg)\\
			& \le \frac{\delta_s}{k} + 2\delta_s + \frac{\delta_s}{k}  \le 3\delta_s ~~~~ (\text{since } k \ge 2)
		\end{align*}
		
		This consequently implies that for any sup-phase $s \ge r$, $\E[|\cA_{r,s}|] \le {3\delta_s}\E[|\cA_{r,s-1}|]$.
		Then applying Markov's Inequality we get:
		
		\begin{align*}
			Pr\Bigg( |\cA_{r,s}| \le \frac{2}{19}|\cA_{r,s-1}| \Bigg)  \le \frac{3\delta_s|\cA_{r,s-1}|}{\frac{2}{19}|\cA_{r,s-1}|} = \frac{57\delta_s}{2}
		\end{align*}
		
		Finally applying union bound over all sub-phases $s= 1,2,\ldots$, and all $r = 1,2, \ldots s$, we get: 
		
		\begin{align*}
			\sum_{s = 1}^{\infty}\sum_{r = 1}^{s}\frac{57\delta_s}{2} = \sum_{s = 1}^{\infty}s\frac{57\delta}{240s^3} = \frac{57\delta}{240}\sum_{s = 1}^{\infty}\frac{1}{s^2} \le \frac{57\delta}{240}\frac{\pi^2}{6} \le \frac{57\delta}{120} \le \frac{19\delta}{20}.
		\end{align*}
		
	\end{proof}
	
	%***************************************************
	
	Thus combining Lem. \ref{lem:bistaystf} and \ref{lem:nbigoestf}, we get that the total failure probability of \algfewf\, is at most $\frac{\delta}{20} + \frac{19\delta}{20} = \delta $.
	
	The remaining thing is to prove the sample complexity bound which crucially follows from a similar claim as proved in Lem. \ref{lem:sc_item}. As before, at any sub-phase $s$, we call the item $b_s$ as the pivot element of phase $s$, then
	
	\begin{restatable}[]{lem}{scitemtf}
		\label{lem:sc_itemtf}
		Assume both Lem. \ref{lem:bistaystf} and Lem. \ref{lem:nbigoestf} holds good and the algorithm does not do a mistake. Consider any item $i \in [n]_r$, for any $r = 1,2, \ldots \log_2(\Delta_{\min})$. Then the total number of times item $i$ gets played as a non-pivot item (i.e. appear in at most one of the $k$-subsets per sub-phase $s$) during the entire run of Alg. \ref{alg:fetf} is $O\Big( \frac{(2^r)^2\thetk}{m}\ln \frac{rk}{\delta}  \Big)$. %\red{Check}
	\end{restatable}
	
	\begin{proof}
		Let us denote the sample complexity of item $i$ (as a non-pivot element) from phase $x$ to $y$ as $\cN^{(i)}_{x,y}$, for any $1 \le x < y < \infty$. Additionally, recalling from Lem. \ref{lem:algs} that $\thetsh \le 7\thetk$, we now prove the claim with the following two case analyses:
		
		\textbf{(Case 1)} Sample complexity till sub-phase $s = r-1$: Note that in the worst case item $i$ can get picked at every sub-phase $s = 1,2,\ldots$ $r-1$, and at every $s$ it is played for $t_s$ rounds. Thus the total number of plays of item $i \in [n]_r$ (as a non-pivot item), till sub-phase $r-1$ becomes:
		
		\[
		\cN^{(i)}_{1,r-1} \le \sum_{s = 1}^{r-1}t_s = \sum_{s = 1}^{r-1}\frac{14\thetk}{m\epsilon_s^2}\ln \frac{k}{\delta_s} = \frac{14\thetk}{m4^{-2}}\sum_{s = 1}^{r-1}(2^s)^2\ln \frac{120ks^3}{\delta} = O\Big( \frac{(2^r)^2\thetk}{m}\ln \frac{rk}{\delta}  \Big)
		\]
		
		\textbf{(Case 2)} Sample complexity from sub-phase $s \ge r$ onwards: Assuming Lem. \ref{lem:nbigoestf} holds good, note that if we define a random variable $I_s$ for any sub-phase $s \ge r$ such that $I_s = \1(i \in \cA_s)$, then clearly $\E[I_{s}] \le \frac{2}{19}\E[I_{s-1}]$ (as follows from the analysis of Lem. \ref{lem:bistaystf}). Then the total expected sample complexity of item $i \in [n]_r$ for round $r, r+1, \ldots \infty$ becomes:
		\begin{align*}
			& \cN^{(i)}_{r,\infty}\le \frac{224\thetk}{m}\sum_{s = r}^{\infty}\bigg(\frac{2}{19}\bigg)^{s-r+1}4^s\ln \frac{k}{\delta_s} = \frac{224\thetk(2^r)^2}{m}\sum_{s = 0}^{\infty}\bigg(\frac{2}{19}\bigg)^{s+1}(2^s)^2\ln \frac{120k(s+r)^3}{\delta}\\
			& = \frac{448}{19m}\thetk(2^r)^2\sum_{s = 0}^{\infty}\bigg(\frac{8}{19}\bigg)^{s}\ln \frac{120k(s+r)^3}{\delta} \\
			& \le \frac{448}{19m}\thetk(2^r)^2\Bigg[\ln \frac{120kr}{\delta}\sum_{s = 0}^{\infty}\bigg(\frac{8}{19}\bigg)^{s} + \sum_{s = 0}^{\infty}\bigg(\frac{8}{19}\bigg)^{s}\ln(120ks)\Bigg] =  O\Big( \frac{(2^r)^2\thetk}{m}\ln \frac{rk}{\delta}  \Big)
		\end{align*}
		
		Combining the two cases above we get $\cN^{(i)}_{1,\infty} = O\Big( \frac{(2^r)^2\thetk}{m}\ln \frac{rk}{\delta}\Big)$ as well, which concludes the proof.
	\end{proof}
	
	Following similar notations as $\cN^{(i)}_{x,y}$, we now denote the number of times any $k$-subset $S \subseteq [n]$ played by the algorithm in sub-phase $x$ to $y$ as $\cN^{(S)}_{x,y}$. Then using Lem. \ref{lem:sc_itemtf}, the total sample complexity of the algorithm \algfewf\, (lets call it algorithm $\cA$) can be written as:
	
	\begin{align}
		\label{eq:sc_fetf}
		\nonumber \cN_\cA(0,\delta) & = \sum_{S \subset [n]\mid |S|=k} \sum_{s=1}^{\infty}\1(S \in \{\cB_1,\ldots, \cB_{B_s}\})t_s = \sum_{i \in [n]} \sum_{s=1}^{\infty}\frac{\1(i \in \cA_s\sm\{b_s\})}{k-1}t_s\\
		\nonumber & = \sum_{s=1}^{\infty} \sum_{i \in [n]}\frac{\1(i \in \cA_s\sm\{b_s\})}{k-1}t_s = \sum_{s=1}^{\infty} \sum_{r=1}^{\log_2(\Delta_{\min})}\sum_{i \in [n]_r}\frac{\1(i \in \cA_s\sm\{b_s\})}{k-1}t_s \\
		\nonumber & = \frac{1}{k-1}\sum_{r=1}^{\log_2(\Delta_{\min})}\sum_{i \in [n]_r}\cN^{(i)}_{1,\infty} ~~(\text{ Lem. \ref{lem:sc_item}})\\
		\nonumber & = \frac{1}{k-1}\sum_{r=1}^{\log_2(\Delta_{\min})}\sum_{i \in [n]_r}O\Big( \frac{(2^r)^2\thetk}{m}\ln \frac{rk}{\delta}\Big) = \frac{\thetk}{k-1}\sum_{r=1}^{\log_2(\Delta_{\min})}|[n]_r|O\Big( \frac{(2^r)^2}{m}\ln \frac{rk}{\delta}\Big) \\
		& = O\Big( \frac{\thetk}{k}\sum_{i=2}^{n}\frac{1}{m\Delta_i^2}\ln \big(\frac{k}{\delta} \ln \frac{1}{\Delta_i} \big) \Big),
	\end{align}
	where the last inequality follows since $2^r < \frac{2}{\Delta_i}$ by definition for all $i \in [n]_r$.
	%Finally the last thing to account for is the additional sample complexity incurred due to calling the subroutine \algep\ at every sub-phase $s$. But following the same argument as of Thm. \ref{thm:sc_fewf}, this is taken care of by Thm. \ref{lem:up_algep}. %, which can easily verified to hold good in this case as well. 
	Finally, same as derived in the proof of Thm. \ref{thm:sc_fewf}, the last thing to account for is the additional sample complexity incurred due to calling the subroutine \algep\ and \algs\, at every sub-phase $s$, which is combinedly known to be of $O\bigg(\frac{|\cA_s|\Theta_[k]}{k} \Big( 1,\frac{1}{(m 2^s)^2}\Big)\ln \frac{k}{\delta} \bigg)$ at any sub-phase $s$ (from Thm. \ref{lem:up_algep} and Cor. \ref{cor:algs}). And using a similar summation as shown above over all $s = 1,2,\ldots \infty$, combined with Lem. \ref{lem:nbigoestf} and using the fact that $2^r < \frac{2}{\Delta_i}$, one can show that the total sample complexity incurred due to the above subroutines is at most $\frac{\Theta_{[k]}}{k}\sum_{i = 2}^{n}\max\big(1,\frac{1}{m \Delta_i^2}\big) \log \frac{k}{\delta})$. Considering the above sample complexity added with the one derived in Eqn. \ref{eq:sc_fetf} finally gives the desired $O\bigg(\frac{\thetk}{k}\sum_{i = 2}^n\max\Big(1,\frac{1}{m \Delta_i^2}\Big) \ln\frac{k}{\delta}\Big(\ln \frac{1}{\Delta_i}\Big)\bigg)$ sample complexity bound of Alg. \ref{alg:fetf}.
\end{proof}

\newpage %%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}
\[	Pr\Big( P(b_s, 1) > 1/2 - \epsilon_s \Big) \geq 1 - \delta_s \]
\end{lem}

\begin{restatable}[]{lem}{bistays}
	\label{lem:bistays}
	With high probability of at least $(1-\frac{\delta}{20})$, item $1$ is never eliminated, i.e. $1 \in \cA_s$ for all sub-phase $s$. More formally, at the end of any sub-phase $s= 1,2,\ldots$, $\hp_{1b_s} > \frac{1}{2} - \epsilon_s$.
\end{restatable}


\textbf{Notations.}
Recall that we defined $\Delta_i = P(1,i) - 1/2$ (Sec. \ref{sec:prb_setup}). We further denote $\Delta_{\min} = \min_{i \in [n]\sm\{1\}}\Delta_i$.
We define the set of arms $[n]_r := \{ i \in [n] : \frac{1}{2^r} \le \Delta_i < \frac{1}{2^{r-1}} \}$, and denote the set of surviving arms in $[n]_r$ at $s^{th}$ sub-phase by $\cA_{r,s}$, i.e. $\cA_{r,s} = [n]_r \cap \cA_s$, for all $s = 1,2, \ldots$.

\begin{restatable}[]{lem}{nbigoes}
	\label{lem:nbigoes}
	Assuming that the best arm $1$ is not eliminated at any sub-phase $s = 1,2,\ldots$, then with probability at least $(1-\frac{19\delta}{20})$, for any sub-phase $s \ge r$, $|\cA_{r,s}| \le \frac{2}{19}|\cA_{r,s-1}|$, for any $r = 0,1,2,\ldots \log_2 (\Delta_{\min})$. 
\end{restatable}


\begin{restatable}[]{lem}{scitem}
	\label{lem:sc_item}
	Assume both Lem. \ref{lem:bistays} and Lem. \ref{lem:nbigoes} holds good and the algorithm does not do a mistake. Consider any item $i \in [n]_r$, for any $r = 1,2, \ldots \log_2(\Delta_{\min})$. Then the total number of times item $i$ gets played as a non-pivot item (i.e. appear in at most one of the $k$-subsets per sub-phase $s$) during the entire run of Alg. \ref{alg:fewf} is $O\Big( (2^r)^2\thetk\ln \frac{rk}{\delta}  \Big)$. %\red{Check}
\end{restatable}


==> conclusion.tex <==
\section{Conclusion}
\label{sec:concl}

% \red{@HA - Check carefully } 
In summary, our paper tackles the dueling bandit problem under privacy constraints. The primary focus is on utility-based preference matrices tailored for vast or potentially infinite decision spaces. The paper introduces new differentially private dueling bandit algorithms for active learning, striking a balance between computational efficiency and nearly optimal performance in both private and non-private regret bounds. In particular, for finite decision spaces of size $K$, our algorithm delivers an order-optimal regret bound of $O(\sum_{i=2}^K \log(KT)/\Delta_i + K/\epsilon)$ while maintaining $\epsilon$-DP, as substantiated by matching lower bound analysis. Additionally, we also extended our algorithms to encompass general $d$-dimensional decision spaces with possibly infinite arms, presenting an $\epsilon$-DP regret algorithm with  regret bound of $\tilde O \left(   \frac{d^6}{\kappa \epsilon  } + \frac{ d\sqrt{T}}{\kappa} \right)$. 


\paragraph{Future Directions. } This work leads a primary foundation of learning with preference feedback in a privacy-preserving way. The literature of preference learning being vast \cite{Busa21survey}, there lies several open questions including understanding the problem complexities for dynamic and adversarial environments, incorporating user-level personalization, understanding the regret-vs-privacy tradeoff beyond utility-based preferences, amongst many.



==> lb.tex <==

\section{Lower Bound }
\label{sec:lb}

In this section, we derive an information-theoretic lower bound for \dpdb\ problem for finite decision space $\cD = [K]$. Our derived lower bound in \cref{thm:LB_fin} corroborates the regret upper bound of our proposed algorithm \cref{alg:fin} (see \cref{thm:fin}), proving the optimality of our results. 
\begin{restatable}[Lower Bound]{thm}{regalgfin}
\label{thm:LB_fin}
Let $K$ and $\epsilon$ be such that $K/\epsilon \le T/2$.
For any $(\epsilon,\delta)$ differentially private algorithm $\cA$\, there exist a preference matrix $P$ such that the regret of $\cA$ on $P$ is lower bounded by
  $$\cR_T(\cA) = \Omega\left( \sum_{i = 2}^K \frac{\log T}{\Delta(1,i)} + \frac{K}{\epsilon} \right),$$
where $\Delta(1,i):= P(1,i) - 1/2$ simply defines the `preference gap' of the $i$-th arm against the best (rank-1) arm, item-$1$ in our case.  
\end{restatable}

We defer the proof of \cref{thm:LB_fin} to the \cref{app:lb}.

% \begin{proof}[Proof sketch of \cref{thm:LB_fin}]
% We give a sketch for the proof and provide the full proof in the appendix. First, note that the non-private lower bound follows from existing results in the dueling bandits literature~\cite{saha2021optimal,bengs2022stochastic,Ailon+14,SGinst20}.
% For the private lower bound, the main idea is that for an $\eps$-DP algorithm to check whether arm $i$ is better than arm $j$, it has to pull them roughly $1/\eps$ times if the gap between them is constant. As we have $K$ different arms, this implies that a private algorithm must pull roughly $K/\eps$ times arms which are not optimal, hence incurring this cost. We provide the full proof in \cref{app:lb}.
%     % We define $K$ different preference matrices, each will pick a different best arm. The idea is to show that any DP algorithm has to behave similarly on an input sequence samples from these preference matrices. Therefore, the algorithm must suffer large regret for some of them.

%     % For $\ell \in [k]$, we define the preference matrix:
%     % \begin{equation*}
%     % P^\ell(i,j) = 
%     % \begin{cases}
%     %     3/4     & \text{if } i = \ell \\
%     %     1/4     & \text{if } j = \ell \\
%     %     1/2     & \text{otherwise}         
%     % \end{cases}
%     % \end{equation*}    
% \end{proof}

==> problem.tex <==
\section{Problem Setting and Notation}
\label{sec:problem}

\textbf{Notations. } Let $[n] := \{1,2, \ldots n\}$ for any $n \in \N$. 
% The entries of any $n \times n$ matrix $\M$ is denoted by $\M = [m_{ij}]_{ij \in [K]\times [K]}$. 
Lower case bold letters denote vectors, upper-case bold letters denote matrices.
%For any function $f$, we abbreviate $f(\x)$ as $f_{x}$.
$\I_d$ denotes the $d \times d$ identity matrix for $d \in \N$. For any vector $\x \in \R^d$, $\|\x\|_2$ denotes the $\ell_2$ norm of $\x$.
%and for any matrix $\bA \in \R^{m\times n}$, $\|\bA\|_2$ denotes the frobenius norm of matrix $\bA$. 
We denote by
$\Delta_{n}:= \{\p \in [0,1]^n \mid \sum_{i = 1}^n p_i = 1, p_{i} \ge 0, \forall i \in [n]\}$ denotes the $n$-simplex and $\e_i$ denotes the $i$-th standard basis vector, $i \in [K]$. $\cB_d(r)$ denotes the $d$-dimensional ball of radius $r$ for any $r \in \R_+$. We use $\tO(\cdot)$ notation to hide logarithmic dependencies.


\subsection{Problem Setting} 
\label{subsec:prob}
We consider the problem of designing differentially private effective prediction models through user preferences in an active learning framework: 
consider decision space $\cD \subset \cB_d(1)$. Assume any item $\x \in \R^d$ in the decision space is associated with a reward/score parameter $r(\x) = \w^{*\top} \x$ for some unknown $\w^* \in \R^d$. At each round, the goal of the learner (algorithm designer) is to find the item with the highest rewarding arm $\x^*:= \arg\max_{\x \in \cD}r(\x)$. 

However, the learner only has access to user preferences in an active sequential manner. At each round $t$, the learner is allowed to actively choose a pair of items $(\a_t,\b_t)$, upon which it gets to see a binary preference feedback $o_t \in \{0,1\}$ on the item pair indicating the winner of the dueling pair. Naturally, the arms with higher rewards would have a higher probability of winning, so one way to model the preference feedback could be $o_t \sim \text{Ber}\bign{\sigma(r(\a_t)-r(\b_t))}$, where 
 $\sigma: \R \mapsto [0,1]$ is the logistic link function, i.e. $\sigma(x) = (1+e^{-x})^{-1}$. Thus $\P(o_t=1) = \sigma(r(\a_t)-r(\b_t))$ denotes the probability of $\a_t$ winning over $\b_t$.

%\red{Infinite arm case: } More generally, ... write for infinite arms... 

%\paragraph{Preference Matrix $(\P)$ \cite{Yue+12}.}
%A preference matrix $\P$ defined on a set of items $[K]$ is a $[0,1]^{K \times K}$ matrix such that for any $i,j \in [K]$, the $(i,j)$-th entry of $\P$, i.e. $P(i,j)$, indicates the probability of item $i$ being preferred over item $j$ when the pair $(i,j)$ is played as a duel. $\P$ always satisfies $P(i,j) = 1-P(j,i)$ and $P(i,i) = 0.5$.  We also denote by $\Delta_{ij} = P(i,j)-0.5$ the gap between arm $i$ and $j$ regarding their relative pairwise preferences. Note for any pair $(i,j)$,  $\Delta_{ij} > 0$ implies on an expectation $i$ wins over $j$ (or preferred over $j$), denoted $i \succ j$.

%\textbf{Adversarial setting. } In general we assume the underlying preference sequence $\{\P_t\}_{t = 1}^T$ is chosen adversarilly over time. 
%\textbf{Stochastic setting. } In this setting, the underlying preference matrix is fixed over time, i.e. $\P_t = \P ~\forall t \in [T]$, for some fixed unknown preference matrix $\P \in [0,1]^{n \times n}$. 
%

\paragraph{Differentially Private Dueling Bandit}
\label{sec:obj}
In this paper, our goal is to solve the above duelling bandits problem under the constraint of differential privacy~\cite{DworkMcNiSm06}. In our setting, each user's sensitive data is the preference $o_t$ that the user provides. Following standard definitions of differential privacy in the online setting~\cite{SmithTh13,AgarwalSi17}, 
we use the following definition for our problem:

% %Differential privacy was originally proposed by~\cite{DworkMcNiSm06},
% as a way to formalize the amount of information about the \emph{input}
% of an algorithm, that could be exposed to an adversary observing its
% \emph{output}, no matter what the adversary's side information is. Now in
% the context of our problem setup, the algorithm's input is the sequence of
% pairwise preference feedback. Consequently, we use the following definition of differentially privacy ($\epsilon$-DP):

%\ha{definition is somewhat weak because this is asking each $a_t,b_t$ to be $\epsilon$-DP. We want the whole output $a_1,\dots,a_T$ to be $\epsilon$-DP.}
\begin{defn}[($\epsilon, \delta)$-differentially private dueling bandit]
\label{def:dpdb}
  A dueling bandit algorithm $\cA$ is $(\epsilon, \delta)$-differentially
  private if for all sequences $o_{1:T}$ and $o'_{1:T}$ that
  differs in at most one time step, we have for any possible outcome 
  $S \subseteq \cO$ in the set of all possible outcomes $\cO$:
  %	\[
  	%\pi(a_t \in S \mid a_{1:t-1}, r_{1:t-1})
  	%\leq 
  	%\pi(a_t \in S \mid a_{1:t-1}, r'_{1:t-1})
  	%e^\epsilon + \delta
\begin{align}
\P & (a_t,b_t,\dots,a_T,b_T \in S \mid o_{1:T})
\leq 
e^\epsilon \P(a_t,b_t,\dots,a_T,b_T \in S \mid o'_{1:T})
 + \delta
\label{eq:dp-bandit}
\end{align}
 When $\delta = 0$, the algorithm is said to be \emph{$\epsilon$-DP}.
\end{defn}


Intuitively, this means that changing the preference outcome $o_t$ for any given arm-pair $(a_t,b_t)$, will not have much effect on the algorithm's prediction at time $t$ or later on in the subsequent rounds. \emph{If each $o_t$ is private information or a point associated with a single individual, then the definition above means that the presence or absence of that individual will not affect too much the output of the algorithm. Hence, the algorithm will not reveal any extra information about this individual leading to privacy protection.}
The privacy parameters $(\epsilon, \delta)$ determine the extent/degree to which an individual entry affects the output; lower values of $(\epsilon, \delta)$ imply higher levels of privacy, and in this work we mainly consider the strongest notion of pure $\epsilon$-DP where $\delta=0$.
 
\paragraph{Performance Measure: Regret Minimization Under $(\epsilon,\delta)$-DP}
As motivated in the introduction, we want to address the problem of user privacy in systems that train on choice data, e.g. Recommender systems and Personalized healthcare. 
%
This requires balancing the tradeoff between optimizing the performance of the prediction model, without sacrificing user privacy. 




%To optimize performance we would want to predict better items to each user, i.e. $\x^*$, but also need to do that in a differentially private fashion.
Towards this, a sensible measure of performance could be to design an $(\epsilon,\delta)$-DP Dueling Bandit algorithm $\cA$ which is designed to optimize the total cumulative regret of the algorithm $\cA$ in $T$ rounds, defined as:
%\ha{this should be a function of $P$ as well. The language here is important for the lower bounds as well} - \red{its std, I think its okay to use P precisely in the LB proof}
\begin{align}
\label{eq:reg}
	\cR_T(\cA) := \max_{\x^* \in \cD}\sum_{t=1}^T \bigg(2r(\x^*) - r(\a_t) - r(\b_t) \bigg).
\end{align}
%
\emph{This implies that the algorithm aims to optimize the regret performance (i.e. converge to the optimum item $\x^*$ as quickly as possible), without violating the differential privacy of the users.} We will refer to this problem as Differentially Private Dueling Bandit (\dpdb) in the rest of the paper. 


\section{Preliminaries: Some Useful Concepts} 
\label{sec:prelims}
\iffalse%%%%%%%%%%%%%%%%%%%%%
\paragraph{Dueling Bandits Problem (DB) \citep{Zoghi+14RUCB,Yue+09}.} In the classical $K$-armed dueling bandits setting, the learning proceeds in rounds, where at each time step $t \in \{1,2,\ldots,T\}$, the learner selects a pair of arms $(a_t, b_t)$ and receives the winner of the duel in terms of a binary preference feedback $o_t(a_t,b_t) \sim \text{Ber}(P(a_t,b_t))$, sampled according to an underlying (fixed but unknown) preference matrix $\mathbf{P} \in [0,1]^{K \times K}$. The objective of the learner is to minimize the cumulative regret with respect to a fixed `best' arm in terms of pairwise preferences, as:

\[
\cR_T = \max_{i^* \in [K]} \frac{\tilde P(i^*,a_t) + \tilde P(i^*,b_t)}{2},
\]
where $\tilde P(i,j):= P(i,j) - \frac{1}{2}$, for all $i,j \in [K]$.
\fi%%%%%%%%%%%%%%

 \begin{defn}[$\varepsilon$-net for any set $\cS$~\citep{matouvsek1989construction,vershynin2018high}]
 \label{def:net}	
 Given any set $\cS\subseteq \{x\in \mathbb{R}^d| \|x\|_2\leq 1\}$ we define an $\varepsilon$-net of $\cS$ as a discrete set $\cS^{(\varepsilon)} \subseteq \mathcal{S}$  such that for any $\x \in \mathcal{D}$, there is some $\x'\in \cS^{(\varepsilon)}$ with $\|\x'-\x\|_2 \leq \varepsilon$.
\end{defn}
%
Throughout the paper, we will use the notation $\cS^{(\varepsilon)}$ to denote an $\varepsilon$-net of the set $\cS$. We also use the following standard fact for the size of $\varepsilon$-net for the unit ball.
\begin{rem}
\label{rem:net}
It is well known that if $\cS$ is the unit ball, then it is well known that (see ~\cite[Cor. 4.2.13]{vershynin2018high}), one can always find such a discrete $\varepsilon$-net of $\cS$ of cardinality at most $(\frac{3}{\varepsilon})^{d}+d$. 
\end{rem}

Our algorithms also require the notion of an optimal design, which is used in order to find a representative set of arms that is called the core-set.
 \begin{defn}[G-Optimal Design] \citep{lattimore2020bandit}
 \label{defn:gopt}	
Consider any set $\cD \subseteq \R^d$, and let $\pi: \cD \mapsto [0,1]$ be any distribution on $\cD$ (i.e. $\sum_{\x \in \cD}\pi(\x) = 1$). Let us define:
\[
V(\pi) = \sum_{\x \in \cD}\pi(\x)\x\x^\top, ~~~ 
g(\pi) = \max_{\x \in \cD}\|\x\|^2_{V(\pi)^{-1}}.
\]
In the subfield of statistics called optimal experimental design, the distribution $\pi$ is called a ``design", and the problem of finding a design that minimizes $g$ is called the G-Optimal design problem.
\end{defn}
%
The set $\text{Supp}(\pi)$ denotes the support of the distribution $\pi$ and is sometimes called the \emph{``Core Set"}. The following theorem characterizes the size of the core set and the minimum value of the function $g(\cdot)$.

\paragraph{Kiefer–Wolfowitz Theorem.}\hspace{-5pt}\citep{lattimore2020bandit}
\iffalse%%%%%%%%%%
\begin{theorem}[]
  Assume that $A \subset \mathbb{R}^d$ is compact and $\text{span}(A) = \mathbb{R}^d$. The following are equivalent:
   (1) $\pi^*$ is a minimizer of $g$.
   (2) $\pi^*$ is a maximizer of $f(\pi) = \log \det V(\pi)$.
   (3) $g(\pi^*) = d$.
  Furthermore, there exists a minimizer $\pi^*$ of $g$ such that $|\text{Supp}(\pi^*)| \leq \frac{d(d + 1)}{2}$.
\end{theorem}
\fi%%%%%%%%%%%%%%%%
%
By Kiefer-Wolfowitz lemma, we know that for any compact set $\cD \subseteq \R^d$, such that $\text{span}(\cD) = \R^d$, there exists a minimizer $\pi^*$ of $g$ such that $g(\pi^*) = d$; further the size of the support of $\pi^*$ is $|\text{Supp}(\pi^*)|\leq \frac{d(d+1)}{2}$. Also, finding such G-Optimal designs are computationally efficient for large class of compact sets $\cD$.

\iffalse%%%%%%%%%
\begin{defn}(Core set for $\mathcal{A}$~\cite{lattimore2020bandit})\label{lem:core}
	For any finite set of actions $\mathcal{A}\subset \{x\in \mathbf{R}^d|\|x\|_2\leq 1\}$ that spans $\mathbb{R}^d$, there is a subset $\mathcal{C}$ of size at most $Bd$ that spans $\mathbb{R}^d$, where $B$ is a constant, and a distribution $\pi$ on  $\mathcal{C}$ such that for any $a\in \mathcal{A}$
	\begin{equation}\label{eq:corelemm}
		a^\top \left(\sum_{\alpha \in \mathcal{C}} \pi(\alpha) \alpha \alpha^\top\right)^{-1} a\leq 2d.
	\end{equation}
	Moreover, $\mathcal{C}$ and $\pi$ can be found in polynomial time in $d$.
\end{defn}
\fi%%%%%%%%%%%%%%%%%%

\paragraph{The Binary Tree Mechanism.}
Our algorithms use the binary tree mechanism~\cite{DworkNaPiRo10,ChanShSo11} which is a key tool in differential privacy that allows to privately estimate the running sum of a sequence of $T$ numbers $a_1,\dots,a_T \in [0,1]$. This mechanism has the following guarantees.
%\ha{version for vectors?}\knote{Added a sentence}
\begin{lem}[\cite{DworkNaPiRo10}, Theorem 4.1]
\label{lemma:bt}
    Let $\epsilon \le 1$.  There is an $\epsilon$-DP algorithm ($\BinTr$) that takes a stream of numbers $a_1,a_2,\dots,a_T \in [0,1]$ and outputs $c_1,c_2,\dots,c_T$ such that for all $t \in [T]$ and any $\delta \in (0,1)$, with probability at least $1-\delta$,
    \begin{equation*}
        \Big| c_t - \sum_{i=1}^t a_i \Big| 
        \leq
        \frac{4  \log(1/\delta) \log^{2.5} T}{\epsilon} .
    \end{equation*}
\end{lem}
%\red{inequality? sensitivity?}


==> rel_works.tex <==
\subsection{Related Works} 
\label{sec:relworks}

Over the years, Dueling Bandits has been extensively studied with various objectives and generalizations. This includes analyzing the learning rate under different preference structures like total ordering, transitivity, stochastic triangle inequality \cite{falahatgar_nips, BTM}, utility-based preference structures \cite{ailon2014reducing, Busa_pl, SG18, ChenSoda+18}, and general pairwise preference matrices \cite{CDB, SparseDB, Komiyama+16}. Depending on the underlying preference structure, the learner's performance has been assessed against various benchmarks, including best arm identification \cite{SGwin18, Busa_aaai, falahatgar_nips}, top-set detection \cite{Busa_top, SG19}, ranking \cite{Ren+18, SGrank18}, among others.

Some recent works have explored Dueling Bandits in scenarios involving adversarial sequences of preference matrices \cite{gupta2021optimal, Adv_DB, ADB}, robustness to corruptions \cite{agarwal2021stochastic}, extension to potentially infinite arm sets \cite{S21, ContDB}, and contextual scenarios \cite{CDB, SK21}. Another interesting line of work related to Dueling Bandits is its subsetwise generalization, also known as battling bandits \cite{Ren+18, sui2018advancements, Brost+16, ChenSoda+18}.

Despite the widespread surge of interest in learning from preference feedback, surprisingly there has not been a single work on preserving user preferences in the feedback. But this is absolutely important in any real-world systems where human preferences are used for training AI systems. For example, in recommender systems like Netflix and Youtube, the systems are trained based on human preferences, like click data or watch history. However, there is a dire need to keep such sensitive information private, which is however at risk unless the recommender systems ensure a privacy-preserving model during training. Similarly, in various domains of healthcare systems, e.g. 

